Exploring Length Generalization For Transformer-based Speech Enhancement

Transformer network architecture has proven effective in speech enhancement. However, as its core module, self-attention suffers from quadratic complexity, making it infeasible for training on long speech utterances. In practical scenarios, speech enhancement models are often required to perform on noisy speech at run-time that is substantially longer than the training utterances. It remains a challenge how a Transformer-based speech enhancement model can generalize to long speech utterances. In this paper, extensive empirical studies are conducted to explore the model's length generalization ability. In particular, we conduct speech enhancement experiments on four training objectives and evaluate with five metrics. Our studies establish that positional encoding is an effective instrument to dampen the effect of utterance length on speech enhancement. We first explore several existing positional encoding methods, and the results show that relative positional encoding methods exhibit a better length generalization property than absolute positional encoding methods. Additionally, we also explore a simpler and more effective positional encoding scheme, i.e. LearnLin, that uses only one trainable parameter for each attention head to scale the real relative position between time frames, which learns the different preferences on short- or long-term dependencies of these heads. The results demonstrate that our proposal exhibits excellent length generalization ability with comparable or superior performance than other state-of-the-art positional encoding strategies.

==> MagSMM_1s.tex <==
% \begin{table}[!b]
%     \centering
%     \scriptsize
%     \small
%     % \def\arraystretch{1.05}
%     \def\arraystretch{0.85}
%     \setlength{\tabcolsep}{3.3pt}
%     % \footnotesize	
%     % \caption{Average CSIG scores for each SNR level and the highest CSIG scores are highlighted in boldface.}
%     \caption{Performance evaluation results in terms of PESQ, ESTOI (in \%), CSIG, CBAK, and COVL. All the models are trained (SMM as the training objective) with 1s noisy-clean speech pairs and tested on noisy speech utterances with lengths of 1s, 5s, 10s, 15s, and 20s.}
%     \label{tab:magsmm1s}
%     % \vspace*{0.1in}
%     \begin{tabular}{@{}cl||ccccc@{}}
%         \hline
%          % &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
%          &  & \multicolumn{5}{c}{\textbf{Metrics}}\\  
%         \cline{3-7}
%         Test Len. & Model & PESQ & ESTOI & CSIG & CBAK & COVL\\  
%         % \hline
%         % Objective & Network & -5 & 0 & 5 & 10 & 15 \\
%         % \hline
%         \hline
%         \hline
%         \multirow{10}{*}{1s}
%         & Noisy    & 1.88 & 54.26 & 2.33 & 1.86 & 1.71 \\
%         % \cline{2-7}
%         \cdashline{2-7}
%         & No-Pos       & 2.48 & 67.30 & 3.14 & 2.54 & 2.41  \\
%         & Sinusoidal   & 2.58 & 70.80 & 3.25 & 2.59 & 2.50  \\
%         & BERT-Pos     & 2.57 & 70.53 & 3.23 & 2.59 & 2.49  \\
%         & Gauss-Bias   & 2.53 & 69.28 & 3.19 & 2.56 & 2.45  \\
%         & T5-Bias      & 2.59 & 71.14 & 3.28 & 2.61 & 2.52  \\
%         & TISA         & \textbf{2.61} & 71.13 & \textbf{3.29} & \textbf{2.62} & \textbf{2.54}  \\
%         & \textcolor{black}{DA-Bias}   & 2.60 & \textbf{71.23} & 3.27 & 2.61 & 2.53  \\
%         & \textcolor{black}{KERPLE}       & 2.58 & 70.60 & 3.25 & 2.60 & 2.51  \\
%         & LearnLin     & 2.59 & 70.82 & 3.27 & 2.61 & 2.53 \\
%         \hline
%         \hline
%         \multirow{10}{*}{5s}
%         & Noisy    & 1.88 & 54.26 & 2.33 & 1.86 & 1.71 \\
%         % \cline{2-7}
%         \cdashline{2-7}
%         & No-Pos       & 2.32 & 64.74 & 2.99 & 2.41 & 2.25  \\
%         & Sinusoidal   & 2.03 & 54.31 & 2.64 & 2.17 & 1.95  \\
%         % & BERT-Pos     & 2.23 & 60.35 & 2.90 & 2.33 & 2.17  \\
%         & BERT-Pos     & 2.02 & 53.19 & 2.64 & 2.14 & 1.94  \\
%         & Gauss-Bias   & 2.38 & 66.33 & 3.06 & 2.47 & 2.32  \\
%         & T5-Bias      & 2.28 & 63.26 & 2.95 & 2.36 & 2.21  \\
%         & TISA         & 2.52 & 70.17 & 3.24 & 2.56 & 2.48  \\
%         & \textcolor{black}{DA-Bias}   & 2.54 & 70.10 & 3.23 & 2.58 & 2.48  \\
%         & \textcolor{black}{KERPLE}       & 2.53 & 70.47 & 3.23 & 2.57 & 2.48  \\
%         & LearnLin     & \textcolor{black}{\textbf{2.57}} & \textcolor{black}{\textbf{71.02}} & \textcolor{black}{\textbf{3.27}} & \textcolor{black}{\textbf{2.60}} & \textcolor{black}{\textbf{2.52}} \\
%         \hline
%         \hline
        
%         \multirow{10}{*}{10s}
%         & Noisy    & 1.92 & 53.19 & 2.40 & 1.87 & 1.75 \\
%         % \cline{2-7}
%         \cdashline{2-7}
%         & No-Pos       & 2.29 & 62.15 & 2.99 & 2.37 & 2.25  \\
%         & Sinusoidal   & 1.93 & 49.85 & 2.53 & 2.06 & 1.87  \\
%         % & BERT-Pos     & 2.11 & 55.51 & 2.79 & 2.22 & 2.07  \\
%         & BERT-Pos     & 1.98 & 50.63 & 2.60 & 2.08 & 1.92  \\
%         & Gauss-Bias   & 2.41 & 64.61 & 3.11 & 2.47 & 2.35  \\
%         & T5-Bias      & 2.22 & 58.75 & 2.89 & 2.26 & 2.14  \\
%         & TISA         & 2.49 & 67.26 & 3.23 & 2.53 & 2.46  \\
%         & \textcolor{black}{DA-Bias}   & 2.51 & 67.39 & 3.23 & 2.55 & 2.47  \\
%         & \textcolor{black}{KERPLE}       & 2.55 & 68.73 & 3.28 & 2.57 & 2.52  \\
%         & LearnLin     & \textbf{2.59} & \textbf{69.34} & \textbf{3.31} & \textbf{2.60} & \textbf{2.56}  \\
%         \hline
%         \hline
        
%         \multirow{10}{*}{15s}
%         & Noisy        & 1.90 & 52.68 & 2.32 & 1.83 & 1.71 \\
%         \cdashline{2-7}
%         & No-Pos       & 2.23 & 61.31 & 2.89 & 2.30 & 2.17  \\
%         & Sinusoidal   & 1.89 & 47.69 & 2.41 & 1.99 & 1.79  \\
%         % & BERT-Pos     & 2.05 & 53.68 & 2.70 & 2.14 & 1.99  \\
%         & BERT-Pos     & 1.97 & 49.21 & 2.56 & 2.04 & 1.89  \\
%         & Gauss-Bias   & 2.37 & 64.34 & 3.03 & 2.43 & 2.30  \\
%         & T5-Bias      & 2.16 & 57.07 & 2.78 & 2.21 & 2.06  \\
%         & TISA         & 2.42 & 65.80 & 3.09 & 2.44 & 2.35  \\
%         & \textcolor{black}{DA-Bias}   & 2.45 & 66.46 & 3.12 & 2.48 & 2.39  \\
%         & \textcolor{black}{KERPLE}       & 2.51 & 68.46 & 3.20 & 2.52 & 2.45  \\
%         & LearnLin     & \textcolor{black}{\textbf{2.56}} & \textcolor{black}{\textbf{69.28}} & \textcolor{black}{\textbf{3.24}} & \textcolor{black}{\textbf{2.56}} & \textcolor{black}{\textbf{2.49}}  \\
%         \hline
%         \hline
        
%         \multirow{10}{*}{20s}
%         & Noisy        & 1.91 & 51.42 & 2.36 & 1.82 & 1.72    \\
%         % \cline{2-7}
%         \cdashline{2-7}
%         & No-Pos       & 2.25 & 59.86 & 2.95 & 2.33 & 2.21  \\
%         & Sinusoidal   & 1.90 & 45.30 & 2.41 & 1.96 & 1.78  \\
%         % & BERT-Pos     & 2.03 & 51.56 & 2.70 & 2.12 & 1.99  \\
%         & BERT-Pos     & 1.97 & 47.42 & 2.52 & 2.02 & 1.86  \\
%         & Gauss-Bias   & 2.41 & 63.43 & 3.11 & 2.45 & 2.35  \\
%         & T5-Bias      & 2.17 & 54.68 & 2.78 & 2.18 & 2.05  \\
%         & TISA         & 2.41 & 63.25 & 3.11 & 2.43 & 2.35  \\
%         & \textcolor{black}{DA-Bias}   & 2.46 & 64.55 & 3.16 & 2.48 & 2.41  \\
%         & \textcolor{black}{KERPLE}       & 2.54 & 67.35 & 3.26 & 2.55 & 2.49  \\
%         & LearnLin     & \textcolor{black}{\textbf{2.58}} & \textcolor{black}{\textbf{68.13}} & \textcolor{black}{\textbf{3.31}} & \textcolor{black}{\textbf{2.59}} & \textcolor{black}{\textbf{2.54}}  \\
%         \hline
%     \end{tabular}
%     \vspace{-1.0em}
% \end{table}



\begin{table}[!t]
    \centering
    \scriptsize
    \small
    % \def\arraystretch{1.05}
    \def\arraystretch{0.82}
    \setlength{\tabcolsep}{3.3pt}
    % \footnotesize	
    % \caption{Average CSIG scores for each SNR level and the highest CSIG scores are highlighted in boldface.}
    \caption{Performance evaluation results in terms of PESQ, ESTOI (in \%), CSIG, CBAK, and COVL. All the models are trained (SMM as the training objective) with 1s noisy-clean speech pairs and tested on noisy speech utterances of 1s, 5s, 10s, 15s, and 20s.}
    \label{tab:magsmm1s}
    % \vspace*{0.1in}
    \begin{tabular}{@{}cl||ccccc@{}}
        \hline
         % &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
         &  & \multicolumn{5}{c}{\textbf{Metrics}}\\  
        % \cline{3-7}
        Test Len. & Model & PESQ & ESTOI & CSIG & CBAK & COVL\\  
        % \hline
        % Objective & Network & -5 & 0 & 5 & 10 & 15 \\
        % \hline
        \hline
        \hline
        \multirow{10}{*}{1s}
        & Noisy    & 1.88 & 54.26 & 2.33 & 1.86 & 1.71 \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos       & 2.48 & 67.30 & 3.14 & 2.54 & 2.41  \\
        & Sinusoidal   & 2.58 & 70.80 & 3.25 & 2.59 & 2.50  \\
        & BERT-Pos     & 2.57 & 70.53 & 3.23 & 2.59 & 2.49  \\
        & Gauss-Bias   & 2.53 & 69.28 & 3.19 & 2.56 & 2.45  \\
        & T5-Bias      & 2.59 & 71.14 & 3.28 & 2.61 & 2.52  \\
        & TISA         & \textbf{2.61} & 71.13 & \textbf{3.29} & \textbf{2.62} & \textbf{2.54}  \\
        & \textcolor{black}{DA-Bias}   & 2.60 & \textbf{71.23} & 3.27 & 2.61 & 2.53  \\
        & \textcolor{black}{KERPLE}       & 2.58 & 70.60 & 3.25 & 2.60 & 2.51  \\
        & LearnLin     & 2.59 & 70.82 & 3.27 & 2.61 & 2.53 \\
        \hline
        \hline
        \multirow{10}{*}{5s}
        & Noisy    & 1.88 & 54.26 & 2.33 & 1.86 & 1.71 \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos       & 2.32 & 64.74 & 2.99 & 2.41 & 2.25  \\
        & Sinusoidal   & 2.06 & 55.49 & 2.65 & 2.20 & 1.98  \\
        % & BERT-Pos     & 2.21 & 60.3509 & 2.887 & 2.33 & 2.15  \\
        & BERT-Pos     & 2.02 & 53.19 & 2.64 & 2.14 & 1.94  \\
        & Gauss-Bias   & 2.38 & 66.33 & 3.06 & 2.47 & 2.32  \\
        & T5-Bias      & 2.28 & 63.26 & 2.95 & 2.36 & 2.21  \\
        & TISA         & 2.52 & 70.17 & 3.24 & 2.56 & 2.48  \\
        & \textcolor{black}{DA-Bias}   & 2.54 & 70.10 & 3.23 & 2.58 & 2.48  \\
        & \textcolor{black}{KERPLE}       & 2.53 & 70.47 & 3.23 & 2.57 & 2.48  \\
        & LearnLin     & \textcolor{black}{\textbf{2.57}} & \textcolor{black}{\textbf{71.02}} & \textcolor{black}{\textbf{3.27}} & \textcolor{black}{\textbf{2.60}} & \textcolor{black}{\textbf{2.52}} \\
        \hline
        \hline
        
        \multirow{10}{*}{10s}
        & Noisy    & 1.92 & 53.19 & 2.40 & 1.87 & 1.75 \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos       & 2.29 & 62.15 & 2.99 & 2.37 & 2.25  \\
        & Sinusoidal   & 1.96 & 51.32 & 2.57 & 2.10 & 1.91  \\
        % & BERT-Pos     & 2.110 & 554.5067 & 2.797 & 2.22 & 2.075  \\
        & BERT-Pos     & 1.98 & 50.63 & 2.60 & 2.08 & 1.92  \\
        & Gauss-Bias   & 2.41 & 64.61 & 3.11 & 2.47 & 2.35  \\
        & T5-Bias      & 2.22 & 58.75 & 2.89 & 2.26 & 2.14  \\
        & TISA         & 2.49 & 67.26 & 3.23 & 2.53 & 2.46  \\
        & \textcolor{black}{DA-Bias}   & 2.51 & 67.39 & 3.23 & 2.55 & 2.47  \\
        & \textcolor{black}{KERPLE}       & 2.55 & 68.73 & 3.28 & 2.57 & 2.52  \\
        & LearnLin     & \textbf{2.59} & \textbf{69.34} & \textbf{3.31} & \textbf{2.60} & \textbf{2.56}  \\
        \hline
        \hline
        
        \multirow{10}{*}{15s}
        & Noisy        & 1.90 & 52.68 & 2.32 & 1.83 & 1.71 \\
        \cdashline{2-7}
        & No-Pos       & 2.23 & 61.31 & 2.89 & 2.30 & 2.17  \\
        & Sinusoidal   & 1.93 & 49.53 & 2.47 & 2.04 & 1.84  \\
        % & BERT-Pos     & 2.053 & 532.6875 & 2.670 & 2.14 & 1.998  \\
        & BERT-Pos     & 1.97 & 49.21 & 2.56 & 2.04 & 1.89  \\
        & Gauss-Bias   & 2.37 & 64.34 & 3.03 & 2.43 & 2.30  \\
        & T5-Bias      & 2.18 & 57.16 & 2.79 & 2.21 & 2.08  \\
        & TISA         & 2.42 & 65.80 & 3.09 & 2.44 & 2.35  \\
        & \textcolor{black}{DA-Bias}   & 2.45 & 66.46 & 3.12 & 2.48 & 2.39  \\
        & \textcolor{black}{KERPLE}       & 2.51 & 68.46 & 3.20 & 2.52 & 2.45  \\
        & LearnLin     & \textcolor{black}{\textbf{2.56}} & \textcolor{black}{\textbf{69.28}} & \textcolor{black}{\textbf{3.24}} & \textcolor{black}{\textbf{2.56}} & \textcolor{black}{\textbf{2.49}}  \\
        \hline
        \hline
        
        \multirow{10}{*}{20s}
        & Noisy        & 1.91 & 51.42 & 2.36 & 1.82 & 1.72    \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos       & 2.25 & 59.86 & 2.95 & 2.33 & 2.21  \\
        & Sinusoidal   & 1.94 & 47.61 & 2.48 & 2.02 & 1.84  \\
        % & BERT-Pos     & 2.02 & 50.56 & 2.66 & 2.11 & 1.96  \\
        & BERT-Pos     & 1.97 & 47.42 & 2.52 & 2.02 & 1.86  \\
        & Gauss-Bias   & 2.41 & 63.43 & 3.11 & 2.45 & 2.35  \\
        & T5-Bias      & 2.19 & 55.44 & 2.81 & 2.20 & 2.08  \\
        & TISA         & 2.41 & 63.25 & 3.11 & 2.43 & 2.35  \\
        & \textcolor{black}{DA-Bias}   & 2.46 & 64.55 & 3.16 & 2.48 & 2.41  \\
        & \textcolor{black}{KERPLE}       & 2.54 & 67.35 & 3.26 & 2.55 & 2.49  \\
        & LearnLin     & \textcolor{black}{\textbf{2.58}} & \textcolor{black}{\textbf{68.13}} & \textcolor{black}{\textbf{3.31}} & \textcolor{black}{\textbf{2.59}} & \textcolor{black}{\textbf{2.54}}  \\
        \hline
    \end{tabular}
    \vspace{-1.0em}
\end{table}


==> MagSMM_2s.tex <==
\begin{table}[!t]
    \centering
    \scriptsize
    \small
    % \def\arraystretch{1.05}
    \def\arraystretch{0.82}
    \setlength{\tabcolsep}{3.3pt}
    % \vspace*{-0.1in}
    % \footnotesize	
    % \caption{Average CSIG scores for each SNR level and the highest CSIG scores are highlighted in boldface.}
    \caption{Performance evaluation results in terms of PESQ, ESTOI (in \%), CSIG, CBAK, and COVL. All the models are trained (SMM as the training objective) with 2s noisy-clean speech pairs and tested on noisy speech utterances with lengths of 2s, 5s, 10s, 15s, and 20s.}
    \label{tab:magsmm2s}
    % \vspace*{0.1in}
    \begin{tabular}{@{}cl||ccccc@{}}
        \hline
         % &  & \multicolumn{5}{c}{\textbf{Input SNR (dB)}}\\  
         &  & \multicolumn{5}{c}{\textbf{Metrics}}\\  
        % \cline{3-7}
        Test Len. & Model & PESQ & ESTOI & CSIG & CBAK & COVL\\  
        % \hline
        % Objective & Network & -5 & 0 & 5 & 10 & 15 \\
        % \hline
        \hline
        \hline
        \multirow{10}{*}{2s}
        & Noisy    & 1.88 & 53.94 & 2.36 & 1.87 & 1.74 \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos        & 2.46 & 66.94 & 3.19 & 2.56 & 2.43  \\
        & Sinusoidal    & 2.57 & 70.62 & 3.30 & 2.62 & 2.54  \\
        & BERT-Pos      & 2.59 & 70.69 & 3.32 & 2.63 & 2.56  \\
        & Gauss-Bias    & 2.50 & 67.63 & 3.23 & 2.58 & 2.47  \\
        & T5-Bias       & 2.61 & \textbf{71.62} & \textbf{3.36} & \textbf{2.66} & \textbf{2.59}  \\
        & TISA          & \textbf{2.62} & 71.34 & \textbf{3.36} & \textbf{2.66} & \textbf{2.59}  \\
        & \textcolor{black}{DA-Bias}    & 2.61 & 70.87 & 3.33 & 2.65 & 2.58  \\
        & \textcolor{black}{KERPLE}    & 2.60 & 70.69 & 3.34 & 2.65 & 2.58  \\
        & LearnLin      & 2.61 & 70.88 & 3.35 & \textbf{2.66} & 2.58 \\
        \hline
        \hline
        \multirow{10}{*}{5s}
        & Noisy    & 1.88 & 54.26 & 2.33 & 1.86 & 1.71 \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos       & 2.41 & 66.79 & 3.11 & 2.49 & 2.36  \\
        & Sinusoidal   & 1.93 & 55.00 & 2.35 & 1.96 & 1.74  \\
        % & BERT-Pos     & 2.42 & 66.93 & 3.11 & 2.47 & 2.35  \\
        & BERT-Pos     & 1.97 & 54.71 & 2.27 & 1.95 & 1.71  \\
        & Gauss-Bias   & 2.49 & 68.31 & 3.18 & 2.55 & 2.43  \\
        & T5-Bias      & 2.59 & 71.60 & 3.32 & 2.61 & 2.56  \\
        & TISA         & 2.62 & 72.01 & 3.35 & 2.63 & 2.59  \\
        & \textcolor{black}{DA-Bias}   & 2.58 & 71.26 & 3.32 & 2.62 & 2.55  \\
        & \textcolor{black}{KERPLE}   & 2.61 & 71.84 & 3.32 & 2.62 & 2.56  \\
        & LearnLin     & \textcolor{black}{\textbf{2.63}}& \textcolor{black}{\textbf{72.05}} & \textcolor{black}{\textbf{3.37}}& \textcolor{black}{\textbf{2.65}}& \textcolor{black}{\textbf{2.60}}\\
        \hline
        \hline
        
        \multirow{10}{*}{10s}
        & Noisy    & 1.92 & 53.19 & 2.40 & 1.87 & 1.75 \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos       & 2.36 & 64.03 & 3.11 & 2.46 & 2.35  \\
        & Sinusoidal   & 1.92 & 52.85 & 2.37 & 1.87 & 1.74  \\
        % & BERT-Pos     & 2.29 & 60.44 & 2.99 & 2.35 & 2.23  \\
        & BERT-Pos     & 1.94 & 50.39 & 2.20 & 1.85 & 1.66  \\
        & Gauss-Bias   & 2.51 & 66.89 & 3.25 & 2.55 & 2.48  \\
        & T5-Bias      & 2.56 & 68.69 & 3.31 & 2.59 & 2.55  \\
        & TISA         & 2.59 & 69.43 & 3.37 & 2.61 & 2.59  \\
        & \textcolor{black}{DA-Bias}   & 2.54 & 68.09 & 3.30 & 2.58 & 2.53  \\
        & \textcolor{black}{KERPLE}   & 2.63 & 70.24 & 3.38 & 2.63 & 2.61  \\
        & LearnLin     & \textcolor{black}{\textbf{2.65}} & \textcolor{black}{\textbf{70.51}} & \textcolor{black}{\textbf{3.40}} & \textcolor{black}{\textbf{2.66}} & \textcolor{black}{\textbf{2.63}}  \\
        \hline
        \hline
        
        \multirow{10}{*}{15s}
        & Noisy        & 1.90 & 52.68 & 2.32 & 1.83 & 1.71 \\
        \cdashline{2-7}
        & No-Pos       & 2.31 & 62.89 & 3.01 & 2.38 & 2.26  \\
        & Sinusoidal   & 1.89 & 52.70 & 2.32 & 1.84 & 1.70  \\
        % & BERT-Pos     & 2.19 & 57.46 & 2.86 & 2.26 & 2.13  \\
        & BERT-Pos     & 1.92 & 48.90 & 2.15 & 1.80 & 1.62  \\
        & Gauss-Bias   & 2.46 & 66.24 & 3.17 & 2.50 & 2.42  \\
        & T5-Bias      & 2.47 & 67.23 & 3.18 & 2.49 & 2.43  \\
        & TISA         & 2.51 & 68.27 & 3.25 & 2.53 & 2.49  \\
        & \textcolor{black}{DA-Bias}   & 2.45 & 66.22 & 3.17 & 2.49 & 2.42  \\
        & \textcolor{black}{KERPLE}   & 2.59 & 70.05 & 3.31 & 2.58 & 2.54  \\
        & LearnLin     & \textcolor{black}{\textbf{2.61}} & \textcolor{black}{\textbf{70.35}} & \textcolor{black}{\textbf{3.35}} & \textcolor{black}{\textbf{2.61}} & \textcolor{black}{\textbf{2.58}}  \\
        \hline
        \hline
        
        \multirow{10}{*}{20s}
        & Noisy        & 1.91 & 51.42 & 2.36 & 1.82 & 1.72    \\
        % \cline{2-7}
        \cdashline{2-7}
        & No-Pos       & 2.33 & 61.36 & 3.05 & 2.39 & 2.30  \\
        & Sinusoidal   & 1.90 & 51.23 & 2.36 & 1.83 & 1.72  \\
        % & BERT-Pos     & 2.18 & 54.98 & 2.87 & 2.24 & 2.13  \\
        & BERT-Pos     & 1.93 & 47.69 & 2.16 & 1.79 & 1.62  \\
        & Gauss-Bias   & 2.50 & 65.30 & 3.24 & 2.53 & 2.46  \\
        & T5-Bias      & 2.48 & 65.07 & 3.21 & 2.49 & 2.44  \\
        & TISA         & 2.51 & 66.29 & 3.28 & 2.52 & 2.50  \\
        & \textcolor{black}{DA-Bias}   & 2.43 & 63.36 & 3.17 & 2.47 & 2.40  \\
        & \textcolor{black}{KERPLE}   & 2.62 & 68.93 & 3.38 & 2.62 & 2.60  \\
        & LearnLin      & \textcolor{black}{\textbf{2.64}} & \textcolor{black}{\textbf{69.30}} & \textcolor{black}{\textbf{3.41}} & \textcolor{black}{\textbf{2.64}} & \textcolor{black}{\textbf{2.63}}  \\
        \hline
    \end{tabular}
    \vspace{-0.5em}
\end{table}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

